Towards Unbiased Exploration in Partial Label Learning

We consider learning a probabilistic classifier from partially-labelled supervision (inputs denoted with multiple possibilities) using standard neural architectures with a softmax as the final layer. We identify a bias phenomenon that can arise from the softmax layer in even simple architectures that prevents proper exploration of alternative options, making the dynamics of gradient descent overly sensitive to initialisation. We introduce a novel loss function that allows for unbiased exploration within the space of alternative outputs. We give a theoretical justification for our loss function, and provide an extensive evaluation of its impact on synthetic data, on standard partially labelled benchmarks and on a contributed novel benchmark related to an existing rule learning challenge.

==> app-manyplots.tex <==
%auto-ignore
\section{Learning Curves with Different Random Seeds on the Small Consistent Dataset}
\label{app:small_consistent}

In the body of the paper (in \Cref{subsec:synexp}) we presented
experiments with a small syntactic dataset and provided average
training accuracies over 1000 random network initializations in
\Cref{fig:small_consistent_dataset}.  To provide a qualitative
comparison of the different loss functions on this dataset, we
show $10$ randomly-selected training curves for each loss function.
On all plots, we show how the probabilities of allowed outputs change
during training. In the graphs below, Total refers to the sum of all allowed
probabilities. On this dataset, the only optimal output is $o_0$,
corresponding to the blue curve. In the caption, we provide the number
of times that learning resulted in the optimal output being assigned the
highest probability.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_0.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_1.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_2.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_3.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_4.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_5.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_6.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_7.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_8.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_6_prp_9.png}
  \caption{Change of probabilities of allowed outputs during training
    under the $\prploss$ on the small consistent synthetic
    dataset. The optimal output is selected $10$ times out of $10$ trials.}
  \label{fig:synthetic_small_consistent_prp_seeds}
\end{figure}


\begin{figure}[htb]
  \centering
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_0.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_1.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_2.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_3.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_4.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_5.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_6.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_7.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_8.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_7_nll_9.png}
  \caption{Change of probabilities of allowed outputs during training
    under the $\nllloss$ on the small consistent synthetic
    dataset. The optimal output is selected once out of $10$ trials.}
  \label{fig:synthetic_small_consistent_nll_seeds}
\end{figure}


\begin{figure}[htb]
  \centering
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_0.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_1.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_2.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_3.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_4.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_5.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_6.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_7.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_8.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_20_meritocracy0.75_9.png}
  \caption{Change of probabilities of allowed outputs during training
    under the $\bmeritlossC$ on the small consistent
    synthetic dataset. The optimal output is selected $3$ times out of $10$ trials.}
  \label{fig:synthetic_small_consistent_merit0.75_seeds}
\end{figure}



\begin{figure}[htb]
  \centering
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_0.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_1.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_2.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_3.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_4.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_5.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_6.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_7.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_8.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_19_meritocracy0.5_9.png}
  \caption{Change of probabilities of allowed outputs during training
    under the $\bmeritlossB$ on the small consistent
    synthetic dataset. The optimal output is selected $4$ times out of $10$ trials.}
  \label{fig:synthetic_small_consistent_merit0.5_seeds}
\end{figure}


\begin{figure}[htb]
  \centering
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_0.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_1.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_2.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_3.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_4.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_5.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_6.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_7.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_8.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_18_meritocracy0.25_9.png}
  \caption{Change of probabilities of allowed outputs during training
    under the $\bmeritlossA$ on the small consistent
    synthetic dataset. The optimal output is selected $5$ times out of $10$ trials.}
  \label{fig:synthetic_small_consistent_merit0.25_seeds}
\end{figure}



\begin{figure}[htb]
  \centering
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_0.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_1.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_2.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_3.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_4.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_5.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_6.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_7.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_8.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_17_meritocracy0.0_9.png}
  \caption{Change of probabilities of allowed outputs during training
    under the $\uloss$ on the small consistent
    synthetic dataset. The optimal output is selected $8$ times out of $10$ trials.}
  \label{fig:synthetic_small_consistent_merit0.0_seeds}
\end{figure}



\begin{figure}[htb]
  \centering
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_0.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_1.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_2.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_3.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_4.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_5.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_6.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_7.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_8.png}
  \includegraphics[width=0.18\linewidth]{pictures/probchange_16_rc_9.png}
  \caption{Change of probabilities of allowed outputs during training
    under the $\rcloss$ on the small consistent synthetic
    dataset. The optimal output is selected $3$ times out of $10$ trials.}
  \label{fig:synthetic_small_consistent_rc_seeds}
\end{figure}












